A2BFR: Attribute-Aware Blind Face Restoration

Blind face restoration (BFR) aims to recover high-quality facial images from degraded inputs, yet its inherently ill-posed nature leads to ambiguous and uncontrollable solutions. Recent diffusion-based BFR methods improve perceptual quality but remain uncontrollable, whereas text-guided face editing enables attribute manipulation without reliable restoration. To address these issues, we propose A$^2$BFR, an attribute-aware blind face restoration framework that unifies high-fidelity reconstruction with prompt-controllable generation. Built upon a Diffusion Transformer backbone with unified image-text cross-modal attention, A$^2$BFR jointly conditions the denoising trajectory on both degraded inputs and textual prompts. To inject semantic priors, we introduce attribute-aware learning, which supervises denoising latents using facial attribute embeddings extracted by an attribute-aware encoder. To further enhance prompt controllability, we introduce semantic dual-training, which leverages the pairwise attribute variations in our newly curated AttrFace-90K dataset to enforce attribute discrimination while preserving fidelity. Extensive experiments demonstrate that A$^2$BFR achieves state-of-the-art performance in both restoration fidelity and instruction adherence, outperforming diffusion-based BFR baselines by -0.0467 LPIPS and +52.58% attribute accuracy, while enabling fine-grained, prompt-controllable restoration even under severe degradations.

==> tab/table10.tex <==
\begin{table}[htbp]
 \vspace{-15pt}
  \caption{Quantitative results of VQ and NA comparison on \textit{AttrFace-90K-Test}. \textbf{Best} and \underline{second best} performance are highlighted.}
  \vspace{-8pt}
  \centering 
  \resizebox{0.6\columnwidth}{!}{
    \begin{tabular}[t]{l c c}
\toprule  
Methods/Metrics 
& \quad\quad VQ \upcolor{$\uparrow$}\quad\quad & \quad\quad NA \upcolor{$\uparrow$}\quad\quad \\
\midrule

StableSR~\cite{wang2024exploiting}    
 & 90.48 & 89.07 \\

\quad+ Step1X-Edit~\cite{liu2025step1x}        
 & 92.31 & 88.58 \\

\quad+ Flux.1-Kontext~\cite{labs2025flux}       
 & 95.46 & 91.42 \\

\quad+ Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport}    
 & 95.16 & \underline{91.89} \\

\hdashline

DiT4SR~\cite{duan2025dit4sr}    
 & 93.50 & 89.55 \\

\quad+ Step1X-Edit~\cite{liu2025step1x}       
 & 94.02 & 88.92 \\

\quad+ Flux.1-Kontext~\cite{labs2025flux}       
 & \underline{96.39} & 91.26 \\

\quad+ Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport}    
 & 96.11 & 91.47 \\

\hdashline

\rowcolor{gray!20}\textbf{$\text{A}^\text{2}$BFR (Ours)} 
 & \textbf{96.45} & \textbf{93.07} \\

\bottomrule
\end{tabular}
}
\label{Tab:vqna}
\vspace{-16pt}
\end{table}

==> tab/table6.tex <==
% \begin{table}[t]
%   \caption{Quantitative comparison of different $\alpha$ on a subset of AttrFace-90K datasets.}
%    \vspace{-10pt}
%   \centering
%   \setlength{\tabcolsep}{3.5pt} % 减小列间距
%   \small % 使用较小字体
%   \resizebox{\columnwidth}{!}{
%   \begin{tabular}{l c c c c }
%     \toprule  
%     Metrics
% & AA$\uparrow$ & LPIPS$\downarrow$
% & SSIM$\uparrow$   & ID-Sim$\uparrow$  \\
%     \midrule
%     $\alpha= 0.7$ & 0.64 & 0.0853 & 0.8942 & 0.6695 \\
%     $\alpha= 0.85$ & 0.72 & 0.0862 & 0.8935 & 0.6532 \\
%     $\alpha= 1$ (Flow-Edit) & 0.75 & 0.0904 & 0.8898 & 0.6214 \\
%     \bottomrule
%   \end{tabular}
%   }
%   \vspace{-6pt}
%   \label{Tab:alpha_ae}
% \end{table}


\begin{table}[htbp]
  \caption{Quantitative comparison of different $\alpha$ on a subset of AttrFace-90K datasets.}
  \vspace{-5pt}
  \centering
  \scalebox{0.85}{ % 缩小到85%
    \begin{tabular}{l c c c c}
      \toprule  
      Metrics & $\alpha{=}0.5$ & $\alpha{=}0.7$ & $\alpha{=}0.85$ & $\alpha{=}1$ \\
      \midrule
      AA$\uparrow$ & 0.6167 & 0.6417 & 0.7167 & 0.7500 \\
      ID-Sim$\uparrow$ & 0.6713 & 0.6695 & 0.6532 & 0.6214 \\
      \bottomrule
    \end{tabular}
  }
  \vspace{-5pt}
  \label{Tab:alpha_ae}
\end{table}

==> tab/table7.tex <==
\begin{table}[t]
  \caption{Quantitative comparison of different $\lambda$ for AAL on the subset of AttrFace-90K-Test datasets. \textbf{Best} and \underline{second best} performance are highlighted}
  \centering
  \setlength{\tabcolsep}{4pt}
  \small
  \resizebox{0.7\columnwidth}{!}{
  \begin{tabular}{l c c c c}
    \toprule  
    & \multicolumn{2}{c}{Attribute} & \multicolumn{1}{c}{Fidelity} & Quality \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(l){5-5}
    Methods/Metrics
    & SC $\uparrow$ & AA $\uparrow$
    & LPIPS $\downarrow$  & HyperIQA $\uparrow$ \\
    \midrule
    $\lambda=0$  & 94.46               & 0.6417                 & 0.2889                                      & 0.7829 \\
    $\lambda=0.1$ & 94.68                  & 0.8279                 & 0.2916                                      & 0.7773 \\
    $\lambda=0.2$ & 94.70        &  \textbf{0.8536}     & \underline{0.2863}      & \underline{0.7908} \\
    $\lambda=0.5$ & \underline{94.72}                  & 0.8369                 & \textbf{0.2858}                                        & 0.7819 \\
    $\lambda=0.8$ & \textbf{94.74}                  & \underline{0.8452}                 & 0.2933                                         & \textbf{0.7919} \\
    \bottomrule
  \end{tabular}
  }
  \label{Tab: AAL}
\end{table}


==> tab/table8.tex <==
\begin{table}[t]
  \caption{Quantitative comparison of different $\alpha$ for SDT on the subset of AttrFace-90K-Test datasets. \textbf{Best} and \underline{second best} performance are highlighted.}
  \centering
  \setlength{\tabcolsep}{4pt}
  \small
  \resizebox{0.7\columnwidth}{!}{
  \begin{tabular}{l c c c c c}
    \toprule  
    & \multicolumn{2}{c}{Attribute} & \multicolumn{1}{c}{Fidelity} & Quality \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(l){5-5}
    Methods/Metrics
    & SC $\uparrow$ & AA $\uparrow$
    & LPIPS $\downarrow$ & HyperIQA $\uparrow$ \\
    \midrule
    $\alpha=0$ & \underline{94.77}                  & 0.7757                 & 0.2926                                   & 0.7872 \\
    $\alpha=0.1$ & 94.68                  & 0.8452                & 0.2913                                      & \underline{0.7899}  \\
    $\alpha=0.2$ & 94.70        & 0.8536     & \underline{0.2863}     & \textbf{0.7908} \\
    $\alpha=0.5$ & 94.72                  & \underline{0.8619}                 & \textbf{0.2861}                                     & 0.7808 \\
    $\alpha=0.8$ & \textbf{94.78}                  & \textbf{0.8786}                 & 0.2874                       & 0.7823 \\
    \bottomrule
  \end{tabular}
  }
  \label{Tab:SDT}
\end{table}


==> tab/table9.tex <==
\begin{table}[t]
  \caption{Quantitative comparison of different CFG scale on the subset of AttrFace-90K-Test datasets. \textbf{Best} and \underline{second best} performance are highlighted}
  \centering
  \setlength{\tabcolsep}{4pt}
  \small
  \resizebox{0.7\columnwidth}{!}{
  \begin{tabular}{l c c c c }
    \toprule  
    & \multicolumn{2}{c}{Attribute} & \multicolumn{1}{c}{Fidelity} & Quality \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(l){5-5}
    Methods/Metrics
    & SC $\uparrow$ & AA $\uparrow$
    & LPIPS $\downarrow$ & HyperIQA $\uparrow$ \\
    \midrule
    $CFG=1.0$ & 94.34 & 0.6833 & 0.2973  & 0.6447 \\
    $CFG=3.5$ & \textbf{94.84} & 0.8167 & \textbf{0.2843}  & 0.7876 \\
    $CFG=5.5$ & 94.70 & \textbf{0.8536} & \underline{0.2863}  & \textbf{0.7908} \\
    $CFG=7.5$ & \underline{94.76} & 0.8083 & 0.2939  & 0.7893 \\
    $CFG=10.5$ & 94.73 & \underline{0.8333} & 0.2944  & \underline{0.7886} \\
    \bottomrule
  \end{tabular}
  }
  \label{Tab:CFG_ablation}
\end{table}

